Sustainable Cooperation in Peer-To-Peer Networks

Traditionally, peer-to-peer systems have relied on altruism and reciprocity. Although incentive-based models have gained prominence in new-generation peer-to-peer systems, it is essential to recognize the continued importance of cooperative principles in achieving performance, fairness, and correctness. The lack of this acknowledgment has paved the way for selfish peers to gain unfair advantages in these systems. As such, we address the challenge of selfish peers by devising a mechanism to reward sustained cooperation. Instead of relying on global accountability mechanisms, we propose a protocol that naturally aggregates local evaluations of cooperation. Traditional mechanisms are often vulnerable to Sybil and misreporting attacks. However, our approach overcomes these issues by limiting the benefits selfish peers can gain without incurring any cost. The viability of our algorithm is proven with a deployment to 27,259 Internet users and a realistic simulation of a blockchain gossip protocol. We show that our protocol sustains cooperation even in the presence of a majority of selfish peers while incurring only negligible overhead.

==> sections/oud/1a_introduction.tex <==
% ------------ \\
% -- Peer-to-peer/Decentralized systems rely on reciprocity and altrusim in its core. Even if they focus a lot on incentives  \\
% -- Example: Blockchains require unbiased transaction and block sharing to operate correctly in the network, have fair competition and utility to clients. \\ 
% -- We consider the problem of dealing with malicious or selfish peers that that violate the requirement for the unbiased and fair network infrastructure. 
% This includes the behavior of peers such as freeriding on network, censorship or spam. \\ 
% -- We approach the problem by exchanging the information about the subjective \textit{usefullness} of peers. Instead of enforcing a costly Proof of Service, or fully preventing these attacks we consider slow service starvation of peers that consistently violate the fair network policy \\
% -- The above is achieved using a local scoring of the peer's usefulness and exchange of opinion between each other in a Sybil-tolerant and whitewashing-resistant. \\
% ------------

Peer-to-peer systems fundamentally hinge on the principles of altruism and reciprocity to ensure their functionality and stability. This phenomenon is often by design and allows one to overcome the hurdles imposed by the traditional client-server model, in which a central party ensures the health of the system by providing services. In a decentralized setting, in particular, in peer-to-peer systems, clients must provide services for each other for the overall protocol to function as expected. A prime example of this is the BitTorrent~\cite{bittorent} protocol, which illustrates how availability is maintained through reciprocal altruism. From a protocol point of view availability and performance are completely dependent on the generosity of fellow clients within the network. Of course, from a game theory perspective, the most rational action for clients is to aid in the sharing of data within the network, as it may lead to increased availability of data they aim to acquire. However, as it is a decentralized system, no such guarantees can be given. As such, greedy clients or \textit{free-riders} are not directly incentivized to aid in the overall health of the network. The emergence of paid seedboxes already brought issues within this reciprocal altruistic system to light. As their mere existence indicates that without the---in this instance monetary---incentives present, the quality of service that clients expect cannot be guaranteed.

In contrast to older systems, the new generation of peer-to-peer networks, such as Bitcoin, Ethereum, and IPFS rely on incentives for the correct operation of the network. Despite the heavy focus of researchers and developers on incentives~\cite{incentivessurvey2023}, in their basis, these networks continue to rely on altruism and reciprocity on the network level. 
For instance, the protocol of Bitcoin relies on unbiased transaction- and block-sharing mechanisms. Malicious clients can easily divert from the protocol's rules and diminish the overall quality of service. A challenge within these systems is thus addressing the issue of malicious or \textit{selfish peers} that undermine the unbiased nature of the network through various nefarious tactics. For instance, clients can engage in selfish mining attacks in which they maximize their gain by wasting the resources of others~\cite{eyal2018majority,negy2020selfish}. 


Previously proposed mechanisms leave a lot to be desired. A simple approach based on direct reciprocity, such as the tit-for-tat strategy~\cite{titfortat1981}, is too limited to apply to peer-to-peer systems as it would require an interaction with a client before any kind of reputation metric can be applied. As such interactions cannot be assumed in every system, this would lead to either a very limited view of reputation in a network or network-wide communication to connect with and evaluate every node.
Attempts such as PeerReview~\cite{peerreview} and LiFTinG~\cite{lifting2010} show promising results, although they introduce hefty overheads by analyzing all outgoing and incoming messages or interactions with all peers within the network. Prior scientific work failed to address the phenomena that it is trivial to re-enter the collaborative network under a new identity after abuse, on a large scale known as the Sybil attack~\cite{douceur2002sybil}.

Attempts such as PeerReview~\cite{peerreview} and LiFTinG~\cite{lifting2010} show promising results, although introduce hefty overheads by analyzing all outgoing and incoming messages or interactions with all peers within the network. Prior scientific work failed to address the phenomena that it is trivial to re-enter the collaborative network under a new identity after abuse, on a large scale known as the Sybil attack~\cite{douceur2002sybil}. 

As such, there is a need for an accountability mechanism that is able to function in any type of peer-to-peer system without introducing unnecessary heavy overhead or complexities. For this, we propose a system that is based on an evolutionary mechanism referred to as \textit{indirect reciprocity}~\cite{nowak2005evolution,schmid2021unified}. We believe that this cooperation mechanism is applicable to peer-to-peer systems, allowing the creation of a universal accountability mechanism through the recording of local reciprocal altruism. 

We claim that \emph{locality} is indispensable to decentralized networking for cooperation and address the Sybil attack. Our cooperative network with empirical grounding is based on long-term collaboration between participants. Central gatekeepers are by definition not present in a decentralized architecture, therefore no permission is needed to participate. Such permissionless, free-to-join types of open systems are notoriously hard to realize. Here we build upon the principle of only trusting your local networking neighborhood and ignoring distant strangers in the global network.

% We present the first decentralized network for cooperation with experimentally \emph{proven} effectiveness. Our organizing principle is a \enquote{donation system}, where peers continuously help each other by performing work. Pooling donated resources into a single common collective and fairly distributing them is a well-studied unsolved problem. Incentive alignment, misreporting, fraud, abuse, and fake identity creation are some of the underlying issues.

% In 2012?? the impossibility result was published around cooperative networks, that given certain assumptions it is impossible to defend against Sybils [point to actual math rule or something..something...]. In 202x the authors overturned this impossibility result by modifying the underlying assumptions, it is critical to completely ignore untrusted messages for Sybil-resilient trust and cooperation frameworks. 

To mitigate free-riding and promote fair resource allocation, our approach takes into account the contributions made by peers. Instead of depending on a globally verifiable proof mechanism, we rely on local verification and acknowledgments from other participants in the network. However, this solution presents its own set of challenges, as it opens the door to misreporting, a deceptive behavior in which participants provide false or misleading information about their contributions or performance metrics to gain an unfair advantage. The reliance on local verification and acknowledgments also introduce the potential for Sybil attacks~\cite{douceur2002sybil}, wherein peers use fake identities to misreport their contributions and maximize rewards. Even when employing access restriction techniques, malicious peers can still collude and falsely acknowledge non-existent work. To tackle this problem, we propose an approach that involves exchanging information regarding the \textit{subjective contributions} of peers. Furthermore, we evaluate this mechanism through simulations on the Bitcoin and BitTorrent networks and showcase how it rewards well-performing peers based on subjective contributions and handles reputations based on indirect reciprocity.

% In this research, we address the issue of accountability in peer-to-peer systems through usage of \textit{indirect reciprocity}. In summary, we make the following contributions:

% \begin{itemize}
%     \item We present our universally applicable accountability mechanism for peer-to-peer systems 
%     \item We evaluate this mechanism through simulations on the Bitcoin and BitTorrent protocol and showcase how it rewards well-performing peers based on subjective contributions and indirect reciprocity.
% \end{itemize}


==> sections/oud/1b_introduction.tex <==
Decentralized networks represent a paradigm shift in Internet infrastructure, moving towards a decentralized architecture without a single entity in control. The Internet itself is a rare example of collaborative infrastructure, owned by both nobody and everybody.

In 1988 the Local Computer Networking (LCN) research community published work around \enquote{Unslotted Aloha Networks}~\cite{roy1988} and \enquote{The reality of OSI}~\cite{neumann1988}. In the past 35 years, we have deployed networking that is affordable for a significant portion of humanity. Networking offerings consist of mature fiber-to-the-home solutions, ongoing Starlink deployment, and initial sketches of 6G standardization. However, we made little progress on cooperative decentralized infrastructures.

We present the first decentralized network of human cooperation which is specifically designed to avoid concentrations of power and wealth. The collaboration-inducing tit-for-tat strategy inside the BitTorrent protocol undermined the distribution monopoly of the entertainment industry. The Bitcoin protocol failed to provide a stable alternative to the global financial network with systemic bank failures and government bailouts. %We generalise these past efforts.

The networking community proposed numerous protocols in the past decade around security, privacy, money, friendship, trust, and reputation. These decentralized architectures had difficulty scaling to billions of Internet users. Only central platforms with winner-takes-all dynamics have scaled to billions of users (E.g., Google, Facebook, Netflix, and TikTok).
The cardinal unsolved scientific challenge is how to design protocols in which billions of users pool their resources and strangers cooperate successfully.

%
%Networking with security, privacy, and self-sovereign control of your identity and data proved to be a difficult challenge. With PGP and Bitcoin we initiated the first milestones in security, privacy, and autonomy for ordinary citizens.

We present the first decentralized network for cooperation with experimentally \emph{proven} effectiveness. Our organizing principle is a \enquote{donation system}, where peers continuously help each other by performing work. Pooling donated resources into a single common collective and fairly distributing them is a well-studied unsolved problem. Incentive alignment, misreporting, fraud, abuse, and fake identity creation are some of the underlying issues.

Our cooperative network with empirical grounding is based on long-term collaboration between participants. Central gatekeepers are by definition not present in a decentralized architecture, therefore no permission is needed to participate. Such permissionless, free-to-join types of open systems are notoriously hard to realize. Prior scientific work failed to address the phenomena that it is trivial to re-enter the collaborative network under a new identity after abuse, on a large scale known as the Sybil attack.

We claim that \emph{locality} is indispensable to decentralized networking for cooperation and address the Sybil attack.  
In 2012?? the impossibility result was published around cooperative networks, that given certain assumptions it is impossible to defend against Sybils [point to actual math rule or something..something...]. In 202x the authors overturned this impossibility result by modifying the underlying assumptions, it is critical to completely ignore untrusted messages for Sybil-resilient trust and cooperation frameworks. \emph{Here we build upon the principle of only trusting your local networking neighborhood and ignoring distant strangers in the global network}.

We believe the Local Computer Network community has the knowledge, skills, and rich history to solve the problem of cooperative networking. Economists have described the problem of indirect reciprocity in abstract models based on game theory (2020 Nobel Prize in Economics). Economic competition is still the mainstream paradigm: cooperation and work accounting models attract only marginal interest [SEUKEN+PARKES]. Social scientists have studied public goods, commons resource usage, and freeriding. Managing collective resources such as clean air, fishing grounds, and climate, in general, is a pressing unsolved societal problem. The eight rules for the governance of the commons do not apply to cyberspace (2009 Nobel Prize in Economics). Computer scientists published a wealth of new ideas during the first wave of decentralization, starting with P2P client Napster in 1999. The second wave of decentralization started with Bitcoin. % indirect reciprocity (game theory abstracts the fake identity problem away)
% Ostrom is about physical world (real people, real sea,water, and air. Does not include the unique digital aspects)
% P2P community (lived inside the PeerSim DHT fantasy world, never deployed, never industry-grade trust frameworks)
% crypto Bro (only greed, no focus on fundamental infrastructure investments)

==> sections/oud/1c_introduction.tex <==

Decentralized networks represent a paradigm shift in internet infrastructure, moving towards a decentralized architecture built on distributed ledger technologies and peer-to-peer communication protocols. This shift aims to address issues of centralization, privacy, and trust prevalent in traditional internet infrastructure. As a vital component of decentralized networks, cooperation facilitates an environment where participants work together to achieve common goals, such as maintaining network consensus, sharing resources, or enabling decentralized applications.

Cooperation is essential for the efficient functioning of decentralized networks, as it fosters synergies among participants and enhances overall system resilience. Blockchains, for instance, rely on cooperative efforts to share transactions, disseminate blocks, and maintain the integrity of the shared ledger. Incentives play a crucial role in promoting cooperation by ensuring that participants act in a trustworthy manner. For example, Bitcoin rewards miners for creating new blocks and preserving ledger consistency. Similarly, file-sharing networks like Filecoin and Chia incentivize nodes to share disk space or bandwidth, further encouraging cooperative behavior within the system.

Incentive schemes in decentralized networks require complex algorithms to prevent participants from gaming the system. These algorithms are necessary to maintain network security and integrity, but they come at a cost in terms of computational resources, energy consumption, and overall efficiency. 

Remarkably, despite the extensive reliance on incentives, decentralized networks still demand cooperative behavior grounded in reciprocity and goodwill among peers at the network level. Take Bitcoin, for instance, where the protocol implicitly fosters cooperation among nodes by promoting transaction sharing. Upon receiving a new, valid transaction, a node broadcasts it to its peers. Moreover, the network employs a peer-banning mechanism to further reinforce cooperative behavior, allowing nodes to disconnect from peers exhibiting malicious or non-compliant actions. This transaction-sharing process proves crucial for the network's efficient operation, as it ensures rapid transaction propagation, thwarting bad actors' attempts to double-spend or manipulate the system.

However, the current mechanisms in place within the Bitcoin network do not strictly enforce reciprocity. As a result, potential issues such as freeriding or selfish mining may arise, in which participants attempt to exploit the system for their benefit. These problems highlight the limitations of incentive schemes and the need for more robust reciprocity algorithms to ensure cooperation among network participants. As decentralized networks like Bitcoin continue to grow and evolve, developing more efficient and less resource-intensive incentive schemes that can maintain network security and cooperation without imposing excessive overhead on the system is crucial. 

An alternative approach to achieve fair resource allocation is based on social constructs such as trust and reputation, instead of pricing~\cite{satsiou2009reputation,lai2003incentives}.
This approach promotes long-term collaboration between users and has been extensively studied in the context of file-sharing applications such as BitTorrent and Tor.
Despite this, we observe that using a market-based mechanism is often the winning proposition in deployed, decentralized systems.
The key issue is that current solutions for trust-based resource allocation are unsuitable for deployment in open decentralized networks for the following two reasons.
First, existing solutions for trust-based allocations are highly application domain-specific and cannot easily be redeployed within a different application, e.g., as they are using custom parameters.
Second, existing solutions fail to address key threats in open decentralized systems.
Specifically, they fail to address the phenomena that it is often trivial to re-enter the network under a new identity after abuse, manifesting as what is known as the \emph{Sybil Attack}.
As such, the applicability of existing solutions for trust-based resource allocation is limited to deployment in closed systems with well-defined membership.
At the same time, we see that the number of decentralized applications is quickly increasing.
We argue that a universal, efficient, and fair mechanism for resource allocation in open decentralized networks is becoming a pressing issue.


In this work, we present an efficient and fair middleware for the allocation of resources in open decentralized network, named \SystemName.
We treat each system as a \emph{work system}, where peers continuously perform work for each other.
\SystemName{} consists of three key components, as visualized in Figure~\ref{fig:system_model}.
First, we introduce a lightweight distributed ledger that we name \LedgerName{}.
This ledger is capable of securely storing bilateral agreements between peers, and acts as a collective, long-term memory.
Records are shared with other users in the network.
Second, we introduce an efficient reputation algorithm, based on a novel concept we dubbed \emph{duality walks}.
Finally, we provide an architecture for seamless integration of different allocation policies, based on computed trust scores.
The combination of these components yields a mechanism that is resistant to key forms of abuse in decentralized networks, specifically free-riding behaviour and the Sybil Attack.


SPAR is tolerant of Sybil attacks, where an attacker creates multiple fake identities to undermine the reputation system. Each peer subjectively evaluates the helpfulness of other peers during the local interactions. By monitoring and sharing these evaluations, SPAR fosters an environment in which peers are incentivized to maintain a positive reputation within the network. Consequently, this makes it costly for malicious actors to artificially inflate their reputations or attempt to discredit other peers. In addition to Sybil attacks, SPAR effectively addresses other forms of reputation manipulation, such as strategic whitewashing and collusion, further enhancing the robustness of the system.



% - Each peer in SPAR tracks who was helpful during a local interaction. For example, if peer shared transaction which was later added the block, or peer quickly responded to the data request. 

% Consequently, this approach creates a self-sustaining cycle of cooperation, where peers are motivated to consistently engage in honest behavior.



We demonstrate the effectiveness of SPAR through a series of experiments that show it can handle a wide range of collaboration tasks. We show that SPAR enables reliable Bitcoin transaction sharing, and detects free-riding in data-sharing networks. 
